Recursive Graphical Construction of Tadpole-Free Feynman Diagrams and Their Weights in phi^4-Theory

We review different approaches to the graphical generation of the tadpole-free Feynman diagrams of the self-energy and the one-particle irreducible four-point function. These are needed for calculating the critical exponents of the euclidean multicomponent scalar phi^4-theory with renormalization techniques in d=4-epsilon dimensions.

==> feyntex <==
#!/bin/tcsh
rm *.log *.dvi glaum1* *~ 
rm -r /var/texfonts/tfm/adobe/rotis
rm -r /var/texfonts/pk/deskjet/adobe
rm -r /var/texfonts/pk/deskjet/gnu
latex $1
mpost '\mode=deskjet; input glaum1'
latex $1
latex $1
xdvi $1

